Deep Shape Matching

We cast shape matching as metric learning with convolutional networks. We break the end-to-end process of image representation into two parts. Firstly, well established efficient methods are chosen to turn the images into edge maps. Secondly, the network is trained with edge maps of landmark images, which are automatically obtained by a structure-from-motion pipeline. The learned representation is evaluated on a range of different tasks, providing improvements on challenging cases of domain generalization, generic sketch-based image retrieval or its fine-grained counterpart. In contrast to other methods that learn a different model per task, object category, or domain, we use the same network throughout all our experiments, achieving state-of-the-art results in multiple benchmarks.

==> ext-plots.tex <==
\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{figs/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> figs/data/diffusion.tex <==
\pgfplotstableread{
    avgEdg      Edg         avgCrow     Crow        avgEdgCrow  EdgCrow
    4.1         56.99       3.9         51.41       6.8         64.38
    9.2         62.31       8.8         61.61       15.2        67.24
    14.6        63.32       14.0        65.08       23.8        68.07
    20.3        63.76       19.4        65.71       32.7        68.21
    26.2        63.59       25.1        65.99       41.7        67.91
    32.1        63.32       30.8        66.39       50.8        67.61
    38.2        63.28       36.7        66.54       60.0        67.51
    44.3        63.22       42.8        66.68       69.2        67.58
    50.6        63.00       48.9        66.65       78.5        67.49
    56.8        62.74       55.2        66.63       87.7        67.36
	}{\dffsflickr}

==> figs/data/ep_vs_res.tex <==
% w=1, b=20, nofl15k, no q for sketch2sketch and image2image
\pgfplotstableread{
	epoch  	sk2im		sk2sk
	0      	0.2785		0.4974
    1     	0.3856		0.5985
    2     	0.4044		0.6000
    3     	0.4114		0.6018
    4 		0.4114		0.6053
    5		0.4135		0.6064
    10		0.4182		0.6112
    15		0.4193		0.6145
    20		0.4201		0.6152
	}{\flickr}

\pgfplotstableread{
	epoch  	shoes@1		shoes@10	chairs@1	chairs@10	handbags@1	handbags@10
	0      	16.52		58.26		50.52		85.57		26.2		51.2
    1     	24.35		63.48		56.70		93.81		29.2		61.9
    2     	25.22		66.96		63.92		96.91		29.8		59.5
    3     	27.83		65.22		69.07		96.91		31.6		64.3
    4 		28.70		67.83		70.10		96.91		29.8		63.7
    5		32.17		66.09		67.01		96.91		31.0		64.9
    10		32.17		70.43		71.13		96.91		34.5		65.5
    15		29.57		69.57		73.20		96.91		35.7		67.3
    20		28.70		71.30		72.16		96.91		35.1		67.3
	}{\shoeschairs}

\pgfplotstableread{
	epoch  	sk2im@1		sk2skMAP			
	0      	0.0431		0.1968
    1     	0.0738		0.2890
    2     	0.0776		0.2960	
    3     	0.0784		0.3045
    4 		0.0788		0.3079
    5		0.0795		0.3094
    10		0.0855		0.3162
    15		0.0866		0.3190
    20		0.0876		0.3203
	}{\sketchy}

==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}

